XL-HeadTags: Leveraging Multimodal Retrieval Augmentation for the Multilingual Generation of News Headlines and Tags

Millions of news articles published online daily can overwhelm readers. Headlines and entity (topic) tags are essential for guiding readers to decide if the content is worth their time. While headline generation has been extensively studied, tag generation remains largely unexplored, yet it offers readers better access to topics of interest. The need for conciseness in capturing readers' attention necessitates improved content selection strategies for identifying salient and relevant segments within lengthy articles, thereby guiding language models effectively. To address this, we propose to leverage auxiliary information such as images and captions embedded in the articles to retrieve relevant sentences and utilize instruction tuning with variations to generate both headlines and tags for news articles in a multilingual context. To make use of the auxiliary information, we have compiled a dataset named XL-HeadTags, which includes 20 languages across 6 diverse language families. Through extensive evaluation, we demonstrate the effectiveness of our plug-and-play multimodal-multilingual retrievers for both tasks. Additionally, we have developed a suite of tools for processing and evaluating multilingual texts, significantly contributing to the research community by enabling more accurate and efficient analysis across languages.

==> tables/dt.tex <==
\onecolumn
\footnotesize
\begin{center}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}{cccccccccccccc}
\hline
                                            &                                                         & \multicolumn{12}{c}{\textbf{Text}}                                                                                                                                                                                                                                                                                                                                                                                          \\ \cline{3-14} 
\endfirsthead
%
\endhead
%
\hline
\endfoot
%
\endlastfoot
%
                                            &                                                         & \multicolumn{4}{c|}{\textbf{-w/C (K=5)}}                                                                                                       & \multicolumn{4}{c|}{\textbf{-w/C (K=10)}}                                                                                                      & \multicolumn{4}{c}{\textbf{-w/C (K=15)}}                                                                                  \\ \hline
\textbf{Resource}                           & \textbf{Languages}                                      & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \multicolumn{1}{c|}{\textbf{Mtor}}                & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \multicolumn{1}{c|}{\textbf{Mtor}}                & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \textbf{Mtor}                \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}English}    & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.36 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.3}  & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.31} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0.14 & \cellcolor[HTML]{E8E8E8}0.31 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Portuguese}                         & 0.14                         & 0.28                         & 0.12                         & \multicolumn{1}{c|}{0.24}                         & 0.15                         & 0.29                         & 0.14                         & \multicolumn{1}{c|}{0.25}                         & 0.16                         & 0.3                          & 0.12                         & 0.24                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Spanish}    & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.27} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.29} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.14 & \cellcolor[HTML]{E8E8E8}0.29 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Russian}                            & 0.14                         & 0.26                         & 0.08                         & \multicolumn{1}{c|}{0.18}                         & 0.15                         & 0.28                         & 0.1                          & \multicolumn{1}{c|}{0.19}                         & 0.15                         & 0.28                         & 0.09                         & 0.19                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}French}     & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.26} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.27} & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.12 & \cellcolor[HTML]{E8E8E8}0.27 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Mandarin}                           & 0.17                         & 0.3                          & 0.1                          & \multicolumn{1}{c|}{0.2}                          & 0.19                         & 0.32                         & 0.12                         & \multicolumn{1}{c|}{0.2}                          & 0.2                          & 0.34                         & 0.12                         & 0.2                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Arabic}     & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.21} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.25} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.25 \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-8}{*}{High}} & \multicolumn{1}{c|}{All}                                & 0.15                         & 0.3                          & 0.12                         & \multicolumn{1}{c|}{0.24}                         & 0.17                         & 0.32                         & 0.13                         & \multicolumn{1}{c|}{0.25}                         & 0.17                         & 0.32                         & 0.13                         & 0.25                         \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Turkish}    & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.21} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.23} & \cellcolor[HTML]{E8E8E8}0.2  & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.23 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Ukrainian}                          & 0.14                         & 0.26                         & 0.08                         & \multicolumn{1}{c|}{0.17}                         & 0.15                         & 0.28                         & 0.09                         & \multicolumn{1}{c|}{0.19}                         & 0.16                         & 0.28                         & 0.09                         & 0.19                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Bengali}    & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.18} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.17 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.2}  & \cellcolor[HTML]{E8E8E8}0.25 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.2  \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Persian}                            & 0.19                         & 0.32                         & 0.18                         & \multicolumn{1}{c|}{0.25}                         & 0.2                          & 0.33                         & 0.18                         & \multicolumn{1}{c|}{0.25}                         & 0.21                         & 0.35                         & 0.18                         & 0.26                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Nepali}     & \cellcolor[HTML]{E8E8E8}0.22 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.17 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.2}  & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.19 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.23} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.18 & \cellcolor[HTML]{E8E8E8}0.22 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Urdu}                               & 0.18                         & 0.3                          & 0.15                         & \multicolumn{1}{c|}{0.23}                         & 0.2                          & 0.32                         & 0.17                         & \multicolumn{1}{c|}{0.26}                         & 0.21                         & 0.33                         & 0.17                         & 0.26                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Gujarati}   & \cellcolor[HTML]{E8E8E8}0.18 & \cellcolor[HTML]{E8E8E8}0.29 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.16} & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.16 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.19} & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.18 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Hindi}                              & 0.18                         & 0.31                         & 0.15                         & \multicolumn{1}{c|}{0.22}                         & 0.2                          & 0.32                         & 0.16                         & \multicolumn{1}{c|}{0.24}                         & 0.22                         & 0.35                         & 0.18                         & 0.25                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Marathi}    & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.18} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.16 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.19} & \cellcolor[HTML]{E8E8E8}0.2  & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.19 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Telugu}                             & 0.15                         & 0.27                         & 0.12                         & \multicolumn{1}{c|}{0.16}                         & 0.17                         & 0.28                         & 0.14                         & \multicolumn{1}{c|}{0.17}                         & 0.17                         & 0.29                         & 0.14                         & 0.17                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Tamil}      & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.19} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.21} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.14 & \cellcolor[HTML]{E8E8E8}0.19 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Punjabi}                            & 0.16                         & 0.29                         & 0.14                         & \multicolumn{1}{c|}{0.18}                         & 0.18                         & 0.3                          & 0.16                         & \multicolumn{1}{c|}{0.18}                         & 0.19                         & 0.31                         & 0.16                         & 0.19                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Indonesian} & \cellcolor[HTML]{E8E8E8}0.13 & \cellcolor[HTML]{E8E8E8}0.27 & \cellcolor[HTML]{E8E8E8}0.09 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.22} & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.11 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.25} & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.1  & \cellcolor[HTML]{E8E8E8}0.25 \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-14}{*}{Low}} & \multicolumn{1}{c|}{All}                                & 0.18                         & 0.3                          & 0.14                         & \multicolumn{1}{c|}{0.2}                          & 0.2                          & 0.32                         & 0.15                         & \multicolumn{1}{c|}{0.21}                         & 0.2                          & 0.32                         & 0.15                         & 0.21                         \\ \hline
                                            &                                                         & \multicolumn{12}{c}{\textbf{Image}}                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{3-14} 
                                            &                                                         & \multicolumn{4}{c|}{\textbf{-w/I (K=5)}}                                                                                                       & \multicolumn{4}{c|}{\textbf{-w/I (K=10)}}                                                                                                      & \multicolumn{4}{c}{\textbf{-w/I (K=15)}}                                                                                  \\ \hline
\textbf{Resources}                          & \textbf{Languages}                                      & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \multicolumn{1}{c|}{\textbf{Mtor}}                & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \multicolumn{1}{c|}{\textbf{Mtor}}                & \textbf{R2}                  & \textbf{RL}                  & \textbf{Bleu}                & \textbf{Mtor}                \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}English}    & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.28} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.31} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.37 & \cellcolor[HTML]{E8E8E8}0.14 & \cellcolor[HTML]{E8E8E8}0.31 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Portuguese}                         & 0.13                         & 0.27                         & 0.11                         & \multicolumn{1}{c|}{0.23}                         & 0.15                         & 0.29                         & 0.12                         & \multicolumn{1}{c|}{0.23}                         & 0.15                         & 0.29                         & 0.12                         & 0.23                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Spanish}    & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.27} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.29} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.13 & \cellcolor[HTML]{E8E8E8}0.29 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Russian}                            & 0.14                         & 0.27                         & 0.09                         & \multicolumn{1}{c|}{0.18}                         & 0.16                         & 0.28                         & 0.1                          & \multicolumn{1}{c|}{0.2}                          & 0.16                         & 0.28                         & 0.1                          & 0.2                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}French}     & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.25} & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.27} & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.12 & \cellcolor[HTML]{E8E8E8}0.26 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Mandarin}                           & 0.17                         & 0.31                         & 0.11                         & \multicolumn{1}{c|}{0.2}                          & 0.18                         & 0.32                         & 0.11                         & \multicolumn{1}{c|}{0.2}                          & 0.19                         & 0.33                         & 0.12                         & 0.2                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Arabic}     & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.23} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.25} & \cellcolor[HTML]{E8E8E8}0.2  & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.26 \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-8}{*}{High}} & \multicolumn{1}{c|}{All}                                & 0.15                         & 0.3                          & 0.12                         & \multicolumn{1}{c|}{0.23}                         & 0.17                         & 0.32                         & 0.13                         & \multicolumn{1}{c|}{0.25}                         & 0.17                         & 0.32                         & 0.13                         & 0.25                         \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Turkish}    & \cellcolor[HTML]{E8E8E8}0.18 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.14 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.22} & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.16 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.25} & \cellcolor[HTML]{E8E8E8}0.21 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.24 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Ukrainian}                          & 0.15                         & 0.27                         & 0.09                         & \multicolumn{1}{c|}{0.18}                         & 0.17                         & 0.29                         & 0.1                          & \multicolumn{1}{c|}{0.2}                          & 0.16                         & 0.29                         & 0.09                         & 0.19                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Bengali}    & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.17} & \cellcolor[HTML]{E8E8E8}0.22 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.16 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.2}  & \cellcolor[HTML]{E8E8E8}0.23 & \cellcolor[HTML]{E8E8E8}0.34 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.19 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Persian}                            & 0.17                         & 0.3                          & 0.14                         & \multicolumn{1}{c|}{0.21}                         & 0.2                          & 0.33                         & 0.18                         & \multicolumn{1}{c|}{0.25}                         & 0.22                         & 0.35                         & 0.19                         & 0.26                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Nepali}     & \cellcolor[HTML]{E8E8E8}0.22 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.18 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.22} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.18 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.22} & \cellcolor[HTML]{E8E8E8}0.24 & \cellcolor[HTML]{E8E8E8}0.35 & \cellcolor[HTML]{E8E8E8}0.18 & \cellcolor[HTML]{E8E8E8}0.22 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Urdu}                               & 0.19                         & 0.31                         & 0.16                         & \multicolumn{1}{c|}{0.24}                         & 0.21                         & 0.33                         & 0.18                         & \multicolumn{1}{c|}{0.27}                         & 0.21                         & 0.33                         & 0.17                         & 0.26                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Gujarati}   & \cellcolor[HTML]{E8E8E8}0.18 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.16} & \cellcolor[HTML]{E8E8E8}0.2  & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.18} & \cellcolor[HTML]{E8E8E8}0.2  & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.17 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Hindi}                              & 0.18                         & 0.31                         & 0.14                         & \multicolumn{1}{c|}{0.22}                         & 0.22                         & 0.35                         & 0.17                         & \multicolumn{1}{c|}{0.25}                         & 0.21                         & 0.34                         & 0.16                         & 0.25                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Marathi}    & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.27 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.18} & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.3  & \cellcolor[HTML]{E8E8E8}0.15 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.2}  & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.15 & \cellcolor[HTML]{E8E8E8}0.19 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Telugu}                             & 0.13                         & 0.25                         & 0.1                          & \multicolumn{1}{c|}{0.15}                         & 0.15                         & 0.27                         & 0.12                         & \multicolumn{1}{c|}{0.17}                         & 0.16                         & 0.28                         & 0.12                         & 0.17                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Tamil}      & \cellcolor[HTML]{E8E8E8}0.19 & \cellcolor[HTML]{E8E8E8}0.29 & \cellcolor[HTML]{E8E8E8}0.12 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.18} & \cellcolor[HTML]{E8E8E8}0.22 & \cellcolor[HTML]{E8E8E8}0.32 & \cellcolor[HTML]{E8E8E8}0.13 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.2}  & \cellcolor[HTML]{E8E8E8}0.23 & \cellcolor[HTML]{E8E8E8}0.33 & \cellcolor[HTML]{E8E8E8}0.13 & \cellcolor[HTML]{E8E8E8}0.19 \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Punjabi}                            & 0.12                         & 0.26                         & 0.11                         & \multicolumn{1}{c|}{0.14}                         & 0.15                         & 0.28                         & 0.14                         & \multicolumn{1}{c|}{0.17}                         & 0.16                         & 0.29                         & 0.13                         & 0.16                         \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Indonesian} & \cellcolor[HTML]{E8E8E8}0.14 & \cellcolor[HTML]{E8E8E8}0.28 & \cellcolor[HTML]{E8E8E8}0.09 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.24} & \cellcolor[HTML]{E8E8E8}0.16 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.11 & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}0.26} & \cellcolor[HTML]{E8E8E8}0.17 & \cellcolor[HTML]{E8E8E8}0.31 & \cellcolor[HTML]{E8E8E8}0.1  & \cellcolor[HTML]{E8E8E8}0.26 \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-14}{*}{Low}} & \multicolumn{1}{c|}{All}                                & 0.17                         & 0.29                         & 0.13                         & \multicolumn{1}{c|}{0.19}                         & 0.2                          & 0.32                         & 0.15                         & \multicolumn{1}{c|}{0.22}                         & 0.2                          & 0.32                         & 0.14                         & 0.21                         \\ \hline
\caption{\label{table:language-headline-mt5}
mT5
}
\end{longtable}
\end{center}
% \normalsize
\begin{center}
\begin{longtable}{cccccccccccccc}
\hline
                                            &                                                         & \multicolumn{12}{c}{\textbf{Text}}                                                                                                                                                                                                                                                                                                                                          \\ \cline{3-14} 
\endfirsthead
%
\endhead
%
\hline
\endfoot
%
\endlastfoot
%
                                            &                                                         & \multicolumn{4}{c|}{\textbf{-w/C (K=5)}}                                                                                       & \multicolumn{4}{c|}{\textbf{-w/C (K=10)}}                                                                                      & \multicolumn{4}{c}{\textbf{-w/C (K=15)}}                                                                  \\ \hline
\textbf{Resource}                           & \textbf{Languages}                                      & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \multicolumn{1}{c|}{\textbf{FO}}              & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \multicolumn{1}{c|}{\textbf{FO}}              & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \textbf{FO}              \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}English}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Portuguese}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Spanish}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Russian}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}French}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Mandarin}                           &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Arabic}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-8}{*}{High}} & \multicolumn{1}{c|}{All}                                &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Turkish}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Ukrainian}                          &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Bengali}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Persian}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Nepali}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Urdu}                               &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Gujarati}   & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Hindi}                              &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Marathi}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Telugu}                             &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Tamil}      & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Punjabi}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Indonesian} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-14}{*}{Low}} & \multicolumn{1}{c|}{All}                                &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\ \hline
                                            &                                                         & \multicolumn{12}{c}{\textbf{Image}}                                                                                                                                                                                                                                                                                                                                         \\ \cline{3-14} 
                                            &                                                         & \multicolumn{4}{c|}{\textbf{-w/I (K=5)}}                                                                                       & \multicolumn{4}{c|}{\textbf{-w/I (K=10)}}                                                                                      & \multicolumn{4}{c}{\textbf{-w/I (K=15)}}                                                                  \\ \hline
\textbf{Resources}                          & \textbf{Languages}                                      & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \multicolumn{1}{c|}{\textbf{FO}}              & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \multicolumn{1}{c|}{\textbf{FO}}              & \textbf{F3}              & \textbf{F5}              & \textbf{FM}              & \textbf{FO}              \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}English}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Portuguese}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Spanish}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Russian}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}French}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Mandarin}                           &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Arabic}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-8}{*}{High}} & \multicolumn{1}{c|}{All}                                &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\ \hline
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Turkish}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Ukrainian}                          &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Bengali}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Persian}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Nepali}     & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Urdu}                               &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Gujarati}   & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Hindi}                              &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Marathi}    & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Telugu}                             &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Tamil}      & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{Punjabi}                            &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\
\multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}Indonesian} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \multicolumn{1}{c|}{\cellcolor[HTML]{E8E8E8}} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} & \cellcolor[HTML]{E8E8E8} \\ \cline{2-14} 
\multicolumn{1}{c|}{\multirow{-14}{*}{Low}} & \multicolumn{1}{c|}{All}                                &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          & \multicolumn{1}{c|}{}                         &                          &                          &                          &                          \\ \hline
\end{longtable}
\end{center}

